Can These Views Be One Scene? Evaluating Multiview 3D Consistency when 3D Foundation Models Hallucinate

Multiview 3D evaluation assumes that the images being scored are observations of one static 3D scene. This assumption can fail in NVS and sparse-view reconstruction: inputs or generated outputs may contain artifacts, outlier frames, repeated views, or noise, yet still receive high 3D consistency scores. Existing reference-based metrics require ground truth, while ground-truth-free metrics such as MEt3R depend on learned reconstruction backbones whose failure modes are poorly characterized. We study this reliability problem by comparing neural reconstruction priors with classical geometric verification. We introduce \benchmark, a controlled robustness benchmark for multiview 3D consistency, and a parametric family that decomposes neural metrics into backbone, residual, and aggregation components. This family recovers MEt3R and yields variants up to $3\times$ more robust. Our analysis shows that VGGT, MASt3R, DUSt3R, and Fast3R can hallucinate dense geometry and cross-view support for unrelated scenes, repeated images, and random noise. We introduce COLMAP-based metrics that use matches, registration, dense support, and reconstruction failure as failure-aware consistency signals. On real NVS outputs and a structured human study, these metrics achieve up to $4\times$ higher correlation with human judgments than MEt3R.

==> app_toc.tex <==
% ---------------- Appendix-only contents ----------------
\makeatletter

\newif\ifappendixtoc
\appendixtocfalse

% Adjustable formatting knobs
\newlength{\AppendixTocSectionNumWidth}
\newlength{\AppendixTocSubsectionNumWidth}
\newlength{\AppendixTocSubsectionIndent}
\newlength{\AppendixTocParagraphIndent}

\setlength{\AppendixTocSectionNumWidth}{1.8em}
\setlength{\AppendixTocSubsectionNumWidth}{2.8em}
\setlength{\AppendixTocSubsectionIndent}{1.7em}
\setlength{\AppendixTocParagraphIndent}{5.5em}

\newcommand{\appendixcontents}{%
  \section*{Appendix Contents}
  \vspace{-0.75em}
  \begingroup
    \small
    \setlength{\parindent}{0pt}
    \@starttoc{atc}
  \endgroup
  \vspace{0.75em}
}

% Turn on collection after \appendix
\let\oldappendix\appendix
\renewcommand{\appendix}{%
  \oldappendix
  \appendixtoctrue
}

% Save the original LaTeX sectioning command
\let\old@sect\@sect

% Intercept normal \section, \subsection, and \paragraph in the appendix
\def\@sect#1#2#3#4#5#6[#7]#8{%
  \old@sect{#1}{#2}{#3}{#4}{#5}{#6}[#7]{#8}%
  \ifappendixtoc
    \ifnum#2=1\relax
      \addcontentsline{atc}{appsection}%
        {\protect\numberline{\csname the#1\endcsname}#7}%
    \else\ifnum#2=2\relax
      \addcontentsline{atc}{appsubsection}%
        {\protect\numberline{\csname the#1\endcsname}#7}%
    \else\ifnum#2=4\relax
      \addcontentsline{atc}{appparagraph}{#7}%
    \fi\fi\fi
  \fi
}

% Formatting for the appendix contents

% Appendix sections: large, bold, spaced, no dotted leaders
\newcommand*{\l@appsection}[2]{%
  \addvspace{1.0em}%
  \begingroup
    \parindent 0pt
    \rightskip \@pnumwidth\relax
    \parfillskip -\@pnumwidth\relax
    \leavevmode
    \large\bfseries
    \setlength{\@tempdima}{\AppendixTocSectionNumWidth}%
    \advance\leftskip \@tempdima
    \hskip-\leftskip
    #1%
    \nobreak\hfill
    \nobreak
    \hb@xt@\@pnumwidth{\hfil #2}%
    \par
  \endgroup
}

% Appendix subsections: bold, indented, with dotted leaders
\newcommand*{\l@appsubsection}[2]{%
  \addvspace{0.25em}%
  \begingroup
    \parindent 0pt
    \rightskip \@pnumwidth\relax
    \parfillskip -\@pnumwidth\relax
    \leavevmode
    \normalsize\bfseries
    \setlength{\@tempdima}{\AppendixTocSubsectionNumWidth}%
    \advance\leftskip \AppendixTocSubsectionIndent
    \advance\leftskip \@tempdima
    \hskip-\@tempdima
    #1%
    \nobreak
    \leaders\hbox to .6em{\hss.\hss}\hfill
    \nobreak
    \hb@xt@\@pnumwidth{\hfil #2}%
    \par
  \endgroup
}

% Appendix paragraph titles: smaller, lighter, more indented
\newcommand*{\l@appparagraph}[2]{%
  \begingroup
    \parindent 0pt
    \rightskip \@pnumwidth\relax
    \parfillskip -\@pnumwidth\relax
    \leavevmode
    \small\normalfont
    \advance\leftskip \AppendixTocParagraphIndent
    #1%
    \nobreak
    \leaders\hbox to .6em{\hss.\hss}\hfill
    \nobreak
    \hb@xt@\@pnumwidth{\hfil #2}%
    \par
  \endgroup
}

\makeatother
% --------------------------------------------------------
